Evaluating LLMs Capabilities Towards Understanding Social Dynamics

Social media discourse involves people from different backgrounds, beliefs, and motives. Thus, often such discourse can devolve into toxic interactions. Generative Models, such as Llama and ChatGPT, have recently exploded in popularity due to their capabilities in zero-shot question-answering. Because these models are increasingly being used to ask questions of social significance, a crucial research question is whether they can understand social media dynamics. This work provides a critical analysis regarding generative LLM's ability to understand language and dynamics in social contexts, particularly considering cyberbullying and anti-cyberbullying (posts aimed at reducing cyberbullying) interactions. Specifically, we compare and contrast the capabilities of different large language models (LLMs) to understand three key aspects of social dynamics: language, directionality, and the occurrence of bullying/anti-bullying messages. We found that while fine-tuned LLMs exhibit promising results in some social media understanding tasks (understanding directionality), they presented mixed results in others (proper paraphrasing and bullying/anti-bullying detection). We also found that fine-tuning and prompt engineering mechanisms can have positive effects in some tasks. We believe that a understanding of LLM's capabilities is crucial to design future models that can be effectively used in social applications.

==> Sections/evaluation.tex <==
\section{Evaluation}

\subsection{Procedural Generation for annotations}
We used the Amazon mTurk API for creating a survey for each session respectively. For procedural generation, mTurk does not allow review of the created HITs from the web interface. Thus, all operations have to be performed using either the AWS CLI or the aws-shell.  

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Figures/instagram_dataset_comment_stats.pdf}
    \caption{We use a subset of Instagram dataset consisting of 932 sessions. The figure shows the distribution of comments for sessions}
    \label{fig:enter-label}
\end{figure}

\subsubsection{Annotation Filtering}



==> Sections/methodology.tex <==
\section{Methodology}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{Figures/method.pdf}
    \caption{Our method combines fine-tuning phases for structural awareness and reasoning for session understanding with social understanding. The resulting model is able to detect anti-bullying and explain the reasoning behind the behaviour from a bird's-eye view.}
    \label{fig:method}
\end{figure}

\subsection{Problem Setting}
Given a dataset of social media discourse containing text-based conversations, posts, comments, or interactions from various social media platforms, the goal of this research is to develop a framework for identifying individuals who act as mediators within these online discussions. Mediators are defined as individuals who actively contribute to steering conversations in a positive direction, fostering constructive interactions, and counteracting toxic behaviors.

The problem can be formally stated as follows:

\subsubsection{Inputs}
The input dataset $\mathcal{D}$ consists of $N$ instances of social media discourse, where each instance $d_i \in \mathcal{D}$ is represented as a sequence of text tokens. Each instance $d_i$ captures the interactions and conversations of users on social media platforms, involving various topics, themes, and sentiment expressions.

\subsubsection{Outputs}
The objective is to produce the following outputs:

\begin{enumerate}
    \item \textbf{Mediator Identification:} For each instance $d_i$, identify a subset $\mathcal{M}_i \subseteq \mathcal{U}$ of users who exhibit mediator behavior within the discourse. Here, $\mathcal{U}$ represents the set of all users participating in the social media discourse.
    
    \item \textbf{Behavior and Motivation Explanations:} For each identified mediator $u_j \in \mathcal{M}_i$, generate human-interpretable explanations that shed light on the behavior, actions, and motivations of the mediator. These explanations should provide insights into why the mediator engages in positive discourse and the impact of their actions on the conversation.
    
    \item \textbf{Unsupervised Approach Framework:} Develop an unsupervised approach framework that leverages the knowledge encoded in large language models to identify mediators and generate behavior explanations. This framework should incorporate techniques such as data augmentation and fine-tuning to amplify the ability to detect mediator behavior and explain it.
    
    \item \textbf{Human-Interpretable General Behavior Insights:} Extend the framework to provide broader insights into general behavior patterns within the social media discourse. These insights should go beyond mediator identification and explain the overall dynamics of positive interactions and discourse moderation.
    
    \item \textbf{Evaluation Results:} Evaluate the effectiveness of the proposed approach using procedurally generated crowd-sourced surveys as a baseline. Measure the accuracy of mediator identification, the quality of behavior explanations, and the interpretability of general behavior insights.
\end{enumerate}

The ultimate aim is to contribute to a better understanding of online interactions and discourse dynamics by identifying mediators, explaining their behavior, and offering insights into positive engagement patterns within social media discourse.

\subsection{Fine-tuning phases}

Our method divides fine-tuning a pretrained GPT model in two phases. The first phase consists of reasoning and structural understanding. The second phase consists of social understanding. Since our final objective is to use the context of a social media session to detect anti-bullying and explain the aspects and motivation for their behaviour, the first phase is designed to make the model reason about the relationship between different comments in the session. The second phase of the fine-tuning process is designed to understand the behaviour of the comments in a social context. Finally, by combining both of these aspects, our resultant model is able to develop social reasoning by considering the entire session as context.


% Instruct tuning 

% Lora 
Each phase of the fine-tuning process is performed using \textbf{Lo}w \textbf{R}ank \textbf{A}daptation (LoRA) strategy~\cite{hu2021lora}. This strategy allows us to target particular layers in the model for fine tuning. Consider a weight matrix $W_0 \in \mathbb{R}^{m \times n}$ representing the original weights. We introduce a new set of corresponding weights, $A \in \mathbb{R}^{m \times r}$ and $B \in \mathbb{R}^{r \times n}$, where $r << min(m, n)$. Our models' corresponding weight is now $W_0 + AB$. Thus, backpropogating on $A$ and $B$, we can finetune on a significantly smaller number of parameters.


% How do we prevent mode collapse 
Machine learning models are vulnerable to mode collapse and catastrophic forgetting when training on a certain type of data i.e. training on structural understanding might make to model forget about previously learned knowledge in lieu of learning structure. To prevent such a hazard, we use a combination of task specific data and general instruction data. For the instruction data, we make use of Alpaca instructions which are combined with the task data with a certain probability. 

% Structural Understanding 
The primary objective of training an LLM for next-word prediction is to learn the conditional probability distribution of the next word given the context of preceding words. Formally, let \(w_1, w_2, \ldots, w_{n-1}\) be a sequence of \(n-1\) words, and \(w_n\) be the target word to predict. The goal is to learn the probability \(P(w_n | w_1, w_2, \ldots, w_{n-1})\), which captures the likelihood of different words occurring next in the sequence. To train LLMs, large text corpora are used as datasets. These corpora contain a wide variety of sentences and documents, providing diverse linguistic contexts for the model to learn from. Common sources of data include books, articles, websites, and other textual sources. 

For our problem setting, rather than just predicting the next words, we aim to gain an understanding of the relation between different comments. For instance, a comment in a session may target another comment, some common theme between a set of comments, or the relation between another comment and its reply. To glean insight into the target of the comment in terms of its context, reasoning between the structure of the conversation is critical. Unfortunately, the LLM pre-training doesn't consider these relationships specifically and there is no public data related to reasoning at a comment level in social media discourse. Thus, we rely on other general purpose structured data to act as a surrogate to learn structure and reasoning. We use the WikiTableQuestions~\cite{pasupat2015compositional} dataset to infuse intelligence into the model. This dataset consists of a large variety of independent tables, questions based on one of the tables and a corresponding answer. To answer the question, it is vital to use the data in the table. Some answers might require aggregate reasoning. 

% Social Understanding

% PEFT


\subsubsection{Data Augmentation}
We collected data from three sources: (i) WikiTableQuestions, (ii) Instagram sessions, and (iii) 4chan threads. We augment the dataset using various methods to improve the generalizability of the final model. For the Instagram dataset, the augmentations are based on symbolic data, which can be extracted programatically. We also use summary and paraphrases generated by a Llama-based model to improve the augmentations. The augmentations on the 4chan dataset are centered toward reducing order bias for training. 
% TODO explain order bias. 
For phase 2 of our training process, the augmentated datasets are combined in the following combination:
(i) 20\% alpaca dataset (for generalization and preventing mode collapse)
(ii) 40\% augmented Instagram dataset (for social understanding of the Instagram context)
(iii) 40\% augmented bard dataset.

% TODO Illustrate the instagram augmentations in detail
% TODO Illustrate the bard augmentations in detail

\subsection{Social Context Understanding}
Large language models are pretrained mostly on structured and semi-structured texts. Since our motivation is to analyze social media discourse, we compare the capabilities of LLMS to understand informal social media comments. Our hypothesis is that an LLM which understands a comment would be able to paraphrase it. Many comments consist of a single tag to another user, emojis, or a single word e.g., 'lol'. We filter comments which contain at least 5 words. These comments are used for paraphrasing in two scenarios: (i) instruction based paraphrasing, and (ii) exemplar based paraphrasing. Instruction based paraphrasing consists of an Alpaca format prompt where the instruction asks the language model to paraphrase, the input is the text to paraphrase, and the response is generated by the model. 

We use five main metrics to evaluate the quality of generations: (i) BLEU score, (ii) ROGUE score, (iii) Jaccard similarity, (iv) Cosine similarity, and, (v) Semantic similarity. One of the quirks with generation is that in many cases, the LLM's reproduce the provided text verbatim. This leads to an increase in most of the similarity metrics. Thus, we also report the levenshtein distance for each strata. 

\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lllllllll@{}}
\toprule
               &               & \multicolumn{6}{c}{\textbf{Similarity Metrics}}                                                                                                     & \multicolumn{1}{c}{\textbf{Edit Distance}} \\ \cmidrule(lr){3-8}  \cmidrule(lr){9-9}
\textbf{Model} & \textbf{Type} & \textbf{BLEU}          & \textbf{ROUGE-1}       & \textbf{ROUGE-2}       & \textbf{ROUGE-L}       & \textbf{Jaccard}       & \textbf{Semantic}      & \textbf{Levenshtein}                       \\
13B            & exemplar      & \textbf{0.725 (0.352)} & \textbf{0.865 (0.219)} & \textbf{0.801 (0.299)} & \textbf{0.859 (0.230)} & \textbf{0.784 (0.285)} & \textbf{0.917 (0.124)} & 0.157 (0.228)                              \\
13B            & non\_exemplar  & {\ul 0.687 (0.383)}    & {\ul 0.844 (0.248)}    & {\ul 0.777 (0.322)}    & {\ul 0.838 (0.256)}    & {\ul 0.757 (0.310)}    & {\ul 0.915 (0.128)}    & 0.175 (0.260)                              \\
7B             & exemplar      & 0.654 (0.378)          & 0.768 (0.352)          & 0.734 (0.373)          & 0.763 (0.355)          & 0.678 (0.354)          & 0.888 (0.161)          & 0.239 (0.329)                              \\
7B             & non\_exemplar  & 0.182 (0.310)          & 0.270 (0.396)          & 0.239 (0.393)          & 0.265 (0.396)          & 0.211 (0.313)          & 0.604 (0.233)          & \textbf{0.733 (0.351)}                     \\
CHATGPT        & exemplar      & 0.187 (0.258)          & 0.527 (0.219)          & 0.305 (0.264)          & 0.493 (0.225)          & 0.345 (0.233)          & 0.805 (0.127)          & 0.521 (0.211)                              \\
CHATGPT        & non\_exemplar  & 0.084 (0.094)          & 0.456 (0.172)          & 0.197 (0.183)          & 0.410 (0.165)          & 0.264 (0.137)          & 0.795 (0.119)          & {\ul 0.599 (0.145)}                        \\
GPT2           & exemplar      & 0.401 (0.465)          & 0.489 (0.427)          & 0.426 (0.469)          & 0.479 (0.433)          & 0.451 (0.433)          & 0.788 (0.189)          & 0.488 (0.387)                              \\
GPT2           & non\_exemplar  & 0.453 (0.466)          & 0.532 (0.439)          & 0.480 (0.463)          & 0.526 (0.443)          & 0.522 (0.418)          & 0.800 (0.213)          & 0.467 (0.419)                              \\ \bottomrule
\end{tabular}%
}
\caption{Comparison of similarity metrics and the corresponding edit distance for across various language models when paraphrases generated on social media comments are compared with the original comment. Ideal paraphrase should vary from the original comment but keep the meaning intact.}
\label{tbl:understanding-comparison}
\end{table*}

\begin{figure*}
    \centering
    \includegraphics[width=.9\textwidth]{Figures/experiment1.pdf}
    \caption{Semantic similarity against edit distance for paraphrases. ChatGPT shows a promising balance, while Llama based models tend to repeat the text verbatim. Using exemplars shows performance improvements for Llama 2 7B model.}
    \label{fig:similarity-comparison}
\end{figure*}


TODO: Explanantion of the different metrics and their significance 

TODO: Explanation of why we use levenshtein ratio

TODO: Why llama fails / Gain by 7B

TODO: The problem with generations: verbatim copies and non-sense generation.

TODO: Significance of exemplars







\subsection{Session understanding through GPT}

\subsubsection{Session preprocessing}

\subsubsection{Structural fine-tuning}

\subsection{Clustering Explanations}

